DeltaCNN: End-to-End CNN Inference of Sparse Frame Differences in Videos

Convolutional neural network inference on video data requires powerful hardware for real-time processing. Given the inherent coherence across consecutive frames, large parts of a video typically change little. By skipping identical image regions and truncating insignificant pixel updates, computational redundancy can in theory be reduced significantly. However, these theoretical savings have been difficult to translate into practice, as sparse updates hamper computational consistency and memory access coherence; which are key for efficiency on real hardware. With DeltaCNN, we present a sparse convolutional neural network framework that enables sparse frame-by-frame updates to accelerate video inference in practice. We provide sparse implementations for all typical CNN layers and propagate sparse feature updates end-to-end - without accumulating errors over time. DeltaCNN is applicable to all convolutional neural networks without retraining. To the best of our knowledge, we are the first to significantly outperform the dense reference, cuDNN, in practical settings, achieving speedups of up to 7x with only marginal differences in accuracy.

==> figures/mot16-pred/mot16_pred_figure.tex <==
\begin{figure}[pt]
\begin{subfigure}{.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/pred_02.png}
\end{subfigure}%
\begin{subfigure}{.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/pred_03.png}
\end{subfigure}%
\begin{subfigure}{0.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/pred_04.png}
\end{subfigure}%
\begin{subfigure}{0.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/pred_05.png}
\end{subfigure}%

\begin{subfigure}{.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/update_02.png}
\end{subfigure}%
\begin{subfigure}{.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/update_03.png}
\end{subfigure}%
\begin{subfigure}{0.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/update_04.png}
\end{subfigure}%
\begin{subfigure}{0.25\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/mot16-pred/update_05.png}
\end{subfigure}%

\caption{
Results using \ours to accelerate EfficientDet-d1 inference on MOT16. 
The first row shows predicted bounding boxes with \ours (blue) and with the dense reference network (white).
The second row shows how many layers updated each pixel -- brighter areas are updated by more layers than dark areas. 
\todo{use four different scenes here and use a color legend / hot/cold colors} \chengcheng{We can use the jet colormap, and place a vertical jet color map bar on the side to indicate the magnitude.}
}
\label{fig:mot16_pred_update}
\end{figure}

==> figures/update_masks/update_masks_walk_figure.tex <==

\begin{figure}[pt]
% inputs
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame0.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame1.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame2.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame3.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame4.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame5.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame6.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame7.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame49.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/input/walk_frame99.png}
\end{subfigure}%

% masks
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame0.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame1.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame2.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame3.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame4.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame5.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame6.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame7.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame49.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks/walk_frame99.png}
\end{subfigure}%

% densities
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame0.png}
  \caption*{1 (Dense)}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame1.png}
  \caption*{2}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame2.png}
  \caption*{3}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame3.png}
  \caption*{4}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame4.png}
  \caption*{5}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame5.png}
  \caption*{6}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame6.png}
  \caption*{7}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame7.png}
  \caption*{8}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame49.png}
  \caption*{50}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities/walk_frame99.png}
  \caption*{100}
\end{subfigure}%

% masks no dilation
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame0.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame1.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame2.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame3.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame4.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame5.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame6.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame7.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame49.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil/walk_frame99.png}
\end{subfigure}%

% densities no dilation
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame0.png}
  \caption*{1 (Dense)}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame1.png}
  \caption*{2}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame2.png}
  \caption*{3}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame3.png}
  \caption*{4}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame4.png}
  \caption*{5}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame5.png}
  \caption*{6}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame6.png}
  \caption*{7}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame7.png}
  \caption*{8}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame49.png}
  \caption*{50}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil/walk_frame99.png}
  \caption*{100}
\end{subfigure}%

% masks no dilation t0=0.1
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame0.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame1.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame2.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame3.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame4.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame5.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame6.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame7.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame49.png}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/masks_no_dil_t0-0.1/walk_frame99.png}
\end{subfigure}%

% densities no dilation t0=0.1
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame0.png}
  \caption*{1 (Dense)}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame1.png}
  \caption*{2}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame2.png}
  \caption*{3}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame3.png}
  \caption*{4}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame4.png}
  \caption*{5}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame5.png}
  \caption*{6}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame6.png}
  \caption*{7}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame7.png}
  \caption*{8}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame49.png}
  \caption*{50}
\end{subfigure}%
\begin{subfigure}{.1\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/update_masks/walk/densities_no_dil_t0-0.1/walk_frame99.png}
  \caption*{100}
\end{subfigure}%

\caption{HRNet update propagation over the first 8 frames, the 50th and the 100th frame of a walking sequence. First row shows network input. Second and third row display the update mask generated from the network input and the update density averaged over all layer of the network when using dilation on the input mask. Fourth and fifth row display the update mask and average update density without mask dilation. While the input mask contains less active pixels without dilation, the average density is similar over all frames. Due to a particle trail behind the person, the performance is even slightly worse than with the dilated input masks which is better at keeping the updates locally. At the same time, the PCK@0.2 accuracy decreases from 95.8\% with dilated masks to 81.7\% without. 
The sixth and seventh row show the input mask and average density without dilation, but with a lower threshold for the first layer.
While the first few layers process many more pixels than in the first case, the background noise is removed at some point in the network and only has a small impact on the overall update density.
This way, the performance is nearly identical to case two, but the accuracy is only 0.2\% below the first case.
\todo{Should we put parts of this evaluation into the paper? - if so, move majority of this caption into text. I think it is interesting, but way too big. most of it could be explained in short text}}
\label{fig:update_mask_propagation}
\end{figure}
